TrajectoTree: Trajectory Optimization Meets Tree Search for Planning Multi-contact Dexterous Manipulation

Dexterous manipulation tasks often require contact switching, where fingers make and break contact with the object. We propose a method that plans trajectories for dexterous manipulation tasks involving contact switching using contact-implicit trajectory optimization (CITO) augmented with a high-level discrete contact sequence planner. We first use the high-level planner to find a sequence of finger contact switches given a desired object trajectory. With this contact sequence plan, we impose additional constraints in the CITO problem. We show that our method finds trajectories approximately 7 times faster than a general CITO baseline for a four-finger planar manipulation scenario. Furthermore, when executing the planned trajectories in a full dynamics simulator, we are able to more closely track the object pose trajectories planned by our method than those planned by the baselines.

==> frictional_form_closure.tex <==
We ensure that the object will always be stably grasped by the fingers by enforcing frictional form closure across the entire trajectory. A grasp achieves frictional form closure if it can be maintained when subjected to any external wrench on the object, under the assumption that the hand can exert arbitrarily large contact forces \cite{SpringerGrasping}. To check if a grasp satisfies frictional form closure in the high-level planner, we determine if there is a feasible solution to the following linear program \cite{Lynch2017ModernRM}:

\begin{equation}
\begin{aligned}
& \underset{\kappa}{\text{minimize}}
& & 1 \\
& \text{subject to}
& & G(\kappa^T \lambda) = -g_{app}\\
& & & \kappa_i >= 1
\end{aligned}
\end{equation}

To enforce the frictional form closure constraint in the trajectory optimization problem, we add additional dummy variables $\kappa$ and the constraints from the LP.

